MAD: Multi-Alignment MEG-to-Text Decoding

Deciphering language from brain activity is a crucial task in brain-computer interface (BCI) research. Non-invasive cerebral signaling techniques including electroencephalography (EEG) and magnetoencephalography (MEG) are becoming increasingly popular due to their safety and practicality, avoiding invasive electrode implantation. However, current works under-investigated three points: 1) a predominant focus on EEG with limited exploration of MEG, which provides superior signal quality; 2) poor performance on unseen text, indicating the need for models that can better generalize to diverse linguistic contexts; 3) insufficient integration of information from other modalities, which could potentially constrain our capacity to comprehensively understand the intricate dynamics of brain activity. This study presents a novel approach for translating MEG signals into text using a speech-decoding framework with multiple alignments. Our method is the first to introduce an end-to-end multi-alignment framework for totally unseen text generation directly from MEG signals. We achieve an impressive BLEU-1 score on the \textit{GWilliams} dataset, significantly outperforming the baseline from 5.49 to 6.86 on the BLEU-1 metric. This improvement demonstrates the advancement of our model towards real-world applications and underscores its potential in advancing BCI research. Code is available at $\href{https://github.com/NeuSpeech/MAD-MEG2text}{https://github.com/NeuSpeech/MAD-MEG2text}$.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> text/table_abl_dataset.tex <==
\begin{wraptable}{r}{0.5\textwidth}
%\setlength{\columnsep}{1pt} 
\setlength{\tabcolsep}{3.9pt}
%\small
\caption{Different datasets. \textbf{Bold} for higher socres.}
%换成split-1，增加一个表。story, non overlap，字体大小
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}lllllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{4}{c}{BLEU-N (\%) $\uparrow$} & \multicolumn{3}{c}{ROUGE-1 (\%) $\uparrow$}  \\ \cmidrule(lr){2-8}
\multicolumn{1}{c}{}                         & N=1    & N=2    & N=3   & N=4   & F         & P         & R        &                           \\ \midrule
\textit{GWilliams}                          & \textbf{60.3} & \textbf{55.26} & \textbf{51.24} & \textbf{47.78} & \textbf{58.73} & \textbf{60.88} & \textbf{59.76}                       \\
\textit{Schoffelen}                                   & 52.89  & 48.53    & 46.02  & 44.18  & 54.28     & 53.87     & 56.14          \\ \bottomrule

\end{tabular}
}
\vspace{-15pt}
\label{tab:abl_datasets}
\end{wraptable}




==> text/table_score.tex <==
\begin{table*}[t]
\centering
\caption{\label{tb:scores} Evaluation metrics of MEG-to-Text translation under raw waves input. \textcolor{black}{ For a fair comparison, these results has \textit{w/} and \textit{w/o} the teacher-forcing evaluation setting since EEG-to-Text~\cite{wang2022open_aaai_eeg2text} only has teacher-forcing originally. Default is w/o teacher forcing and `\textit{w/ tf}' means with teacher-forcing.} }

\vspace{5pt}
\small
\resizebox{0.95\textwidth}{!}{
\centering
\begin{tabular}{@{}clllllllll@{}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{BLEU-N (\%) $\uparrow$}} & \multicolumn{3}{c}{\textbf{ROUGE-1 (\%)}$\uparrow$} & \multicolumn{1}{c}{\textbf{WER (\%) $\downarrow$}} \\
 \cmidrule(lr){3-6} \cmidrule(lr){7-9} \cmidrule(lr){10-10}
\textbf{Modality} & \textbf{Method} & N=1 & N=2 & N=3 & N=4 & F  & P & R & \\
\midrule
\rowcolor[HTML]{EFEFEF}
Speech & Whisper~\cite{radford2023robust_whisper_model_originalpaper} & 67.79 & 59.15 & 51.97 & 45.78 & 75.90 & 73.53 & 81.24 & 41.21 \\
Noise & NeuSpeech & 0.0 & 0.0 & 0.0 & 0.0 & 2.84 & 23.9 & 1.5 & 99.98 \\
- & random & 4.99 & 1.18 & 0.59 & 0.41 & 4.79 & 5.95 & 5.87 & 132.30 \\
MEG & eeg-to-text~\cite{wang2022open_aaai_eeg2text} & 9.21 & 2.13 & 0.57 & 0.14 & 9.74 & 10.73 & 11.38 & 118.25 \\
MEG & NeuSpeech & 57.68 & 52.76 & 48.84 & 45.42 & 60.24 & 61.86 & 61.92 & 58.89 \\ 
% MEG & NeuSpeech \textit{\textit{w/ pp}} & \textbf{60.3} & \textbf{55.26} & \textbf{51.24} & \textbf{47.78} & \textbf{58.73} & \textbf{60.88} & \textbf{59.76} & \textbf{56.63} \\ 
\midrule
MEG & eeg-to-text~\cite{wang2022open_aaai_eeg2text} \textit{w/ tf} & 21.66 & 9.27 & 3.93 & 1.73 & 20.11 & 22.48 & 18.71 & 95.69 \\
MEG & NeuSpeech \textit{w/ tf} & 78.13 & 71.25 & 64.79 & 58.86 & 81.91 & 80.52 & 83.68 & 25.38 \\
% MEG & NeuSpeech \textit{\textit{w/ pp} tf} & \textbf{80.20} & \textbf{73.27} & \textbf{66.79} & \textbf{60.81} & \textbf{78.62} & \textbf{78.14} & \textbf{79.54} & \textbf{23.42} \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table*}



==> text/table_split_datasets.tex <==
% \begin{wraptable}{l}{0.5\textwidth}
% %\setlength{\columnsep}{1pt} 
% \setlength{\tabcolsep}{8.9pt}
% %\small
% % \vspace{-10pt}
% \caption{Dataset splits.Noise means input model with Gaussian noise. NeuSpeech means our model's generated text. Here, we only shows the BLEU-1 score. Note, for hold-out story and sentences, we used nucleus sampling p=0.25 for generation. }
% %换成split-1，增加一个表。story, non overlap，字体大小
% \centering
% % \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{@{}lllll@{}}
% \toprule
% Hold-out & Noise  & \multicolumn{2}{c}{Generation}  \\ \midrule
% Session                      & 0.0        & 53.16   &                             \\
% Story                        & 0.0      & 6.91     &                            \\
% Sentences                    & 0.0     & 6.54     &                            \\ \bottomrule
% \end{tabular}
% % }
% % \vspace{-20pt}
% \label{tab:abl_splits}
% \end{wraptable}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\caption{Different dataset splits. Noise means input model with Gaussian noise with same length of MEG signal. We shows the BLEU-1 score and an example of generation. underline{Underline} denotes a fuzzy match with similar semantic meanings. Note, for hold-out story and sentences, we used nucleus sampling p=0.25 for generation. }
\begin{tabular}{@{}lllp{9.5cm}@{}}
\toprule
Hold-out                   & Noise                & \multicolumn{2}{l}{Generation and example sentence}                                                                                                                                                                                                                                                             \\ \midrule
\multirow{2}{*}{Session}   & \multirow{2}{*}{0.0} & \multirow{2}{*}{53.16} &  
\textbf{Ground truth}: \underline{something} worth reading worth writing                                                                                                                                                                                                                   \\
                           &                      &                        & 
\textbf{Prediction}: \underline{some} kind of what i sell                                                                                                                                                                                                                                          \\\midrule
\multirow{2}{*}{Story}     & \multirow{2}{*}{0.0} & \multirow{2}{*}{6.91}  &  \textbf{Ground truth}: I looked down and saw he was pointing to another marker just slightly \underline{different from the one we had just left}                                                                                              \\
                           &                      &                        &  
\textbf{Prediction}: It was different from now and it just wasn't working well. \\ \midrule     
\multirow{2}{*}{Sentences} & \multirow{2}{*}{0.0} & \multirow{2}{*}{6.54}  & \textbf{Ground truth}: her first officer \underline{was staring at} his panel                                                                                                                                                                                                                        \\
                           &                      &                        &  
\textbf{Prediction}: he \underline{glared at} allan eyes him and demanding a response but he                                                                                                                                                                                                       \\ \bottomrule
\end{tabular}
\label{tab:abl_splits}
\end{table}
% GWilliams split-2                         & 53.16  & 50.88  & 49.14 & 47.61 & 56.71     & 66.69     & 55.01                        \\
% GWilliams split-3                         & 6.9  & 1.22  & 0.0 & 0.0 & 6.235     & 6.13     & 7.37                        \\

==> text/table_target_abl_splits.tex <==
\begin{wraptable}{l}{0.5\textwidth}
    \centering
    \caption{Transcription results on different splits, where \textbf{bold} denotes a correct match between ground truth and our prediction. \underline{Underline} denotes a fuzzy match with similar semantic meanings.} 
    
    %Performance on word-level EEG features is significantly better as the task is easier. Still, decoding on raw waves could output meaningful results.
    \label{tab:generation_results_splits} 
    
    \footnotesize
    % \setlength{\tabcolsep}{1.9pt}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{p{8cm}}
    % \begin{tabular}{}
         
     \toprule 
     
     \textbf{Hold-out sentences}\\ \midrule
     
     Ground Truth: I looked down and saw he was pointing to another marker just slightly \underline{\textbf{different} from the one we had just left} \\
     % \hline
     Prediction: \underline{It was \textbf{different} from now} and it just wasn't working well. \\\midrule
     \textbf{Hold-out story}\\ \midrule
     
     Ground Truth: Mahogany \textbf{black} curly hair cut short in the typical military style framed a dark skinned face \\
     % \hline
     Prediction: I must admit, this is a great \textbf{black} or cold weather. It had things such as 
    \\\bottomrule
    \end{tabular}
% \vspace{-15pt}
    }
\end{wraptable}
% \colorbox{orange}{\underline{deaths}} 

==> text/table_targets.tex <==
\begin{table}[!t]
    \centering
    \caption{Transcription results on the unseen MEG waves, where \textbf{bold} denotes a correct match between ground truth and our prediction. \underline{Underline} denotes a fuzzy match with similar semantic meanings. 
    \textcolor{black}{
    For a fair comparison, these results \textbf{do not keep} the teacher-forcing evaluation setting as EEG-to-Text~\cite{wang2022open_aaai_eeg2text} and Dewave \cite{duan2023dewave_brain2text}. This means the decoding process can hold on accumulated errors and predicts the next token with model-generated tokens from previous steps.  } More samples are provided in supp.~\ref{supp.more_examples}.
    %Performance on word-level EEG features is significantly better as the task is easier. Still, decoding on raw waves could output meaningful results.
    \label{tab:generation_results} }
    
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{l }
    % \begin{tabular}{}
         
     \toprule 
     
     \textbf{Decoding Results on \textit{GWilliams}~\cite{Gwilliams_2023_dataset_meg_208sensors_27persons_56h}} \\ \midrule
     
     Ground Truth: At best they tales at worst expeditions into macabre realms no healthy mind need ever see \\
     % \hline
     Prediction: \textbf{At best} it is macred \textbf{at worst expeditions into macabre realms no healthy mind need ever see} that \\\midrule
     
     Ground Truth: He turned to regard the pillar still rising behind his house and ran to see what had been done \\
     % \hline
     Prediction: \textbf{He}-\textbf{turned to regard a pillar still rising behind his house and ran} away from...\textbf{to see what had been done}. \\ \midrule\midrule
     \textbf{Decoding Results on \textit{Schoffelen}~\cite{Schoffelen_2019_dataset_meg_273sensor_96person_80h}} \\ \midrule
     
     Ground Truth: Tijdens de rumoerige bespreking beslisten de leden de staking voort te zetten \\
     % \hline
     Prediction: \textbf{Tijdens de rumoerige bespreking beslisten de leden} of \textbf{de staking voort}. \\\midrule
     
     Ground Truth: Op die goede prestatie was helemaal niets af te dingen \\
     % \hline
     Prediction: \textbf{Op die goede prestatie was} naar een varken afkomen van het nieuwe afguk...
     % \\ \midrule\midrule
     % \textbf{Decoding Results on Schoffelen~\cite{Schoffelen_2019_dataset_meg_273sensor_96person_80h}} \\ \midrule
     % Ground Truth: Vincent die beroemde portretten \textbf{geschilderd heeft kon daar helaas niks mee} verdienen\\\cmidrule
     % Prediction: Toen de heil die behoefte het gezellige beroemden \textbf{geschilderd heeft kon daar helaas niks mee} \\\midrule
     
     % Ground Truth: \textbf{kreta dat prachtige stranden heeft is vanwege het massale toerisme veel minder aantrekkelijk}\\\cmidrule
     % Prediction:  \textbf{kreta dat prachtige stranden heeft is vanwege het massale toerisme veel minder aantrekkelijk} de ene te\\ 
     
     % \multirow{2}{*}{(6)} 
     % & Ground Truth: \underline{\textbf{Het is een minder} tijdrovende procedure dan klassieke} animatie. \\
     % \cmidrule{2-2}
     % & Prediction: \underline{\textbf{Het is een minder} tijdadog de jonge prachter ak with one vast.} \\ 
    %  \midrule
    %  \multirow{2}{*}{(6)} 
    %  & Ground Truth: Martyr gets \underline{royally} \textit{screwed} and comes back for more.\\
    %  \cmidrule{2-2}
    %  & Model Output: ydom \underline{aally} \textit{pissed} by is out to more.\\
    
    \\\bottomrule
    \end{tabular}
    }
\end{table}

% \colorbox{orange}{\underline{deaths}} 

==> text/table_targets_comparison.tex <==
\begin{table*}[!t]
    \small
    \centering
    \caption{
    Transcription results comparison with different methods. \textbf{Bold} font means exact match of words. \underline{Underline} for similar but not exact matching. w/ means with. tf means teacher-forcing, pt means pretraining, jt means joint-training. eeg-to-text~\cite{wang2022open_aaai_eeg2text} here is using beam search as the same setting of ours which is described in Sec.~\ref{subsec:implementation details}. More samples are provided in supp.~\ref{supp.more_examples}.
    }
    \label{tab:generation_results_comparison} 
    
    % \vspace{5pt}
    \resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}llp{11cm}@{}}
\toprule
\\ \cmidrule(l){1-3} 
\multicolumn{1}{c}{\multirow{7}{*}{(1)}} & GT                & I seen him since high school maybe twenty years before and we were never buddies in the first place                                                             \\ 
\multicolumn{1}{c}{}                     & NeuSpeech         & \textbf{I seen him since high school} \underline{when I was young}, at least \textbf{before and we were never buddies in} any place.                              \\
\multicolumn{1}{c}{}                     & NeuSpeech w/ tf   & \textbf{i seen him since high school} when even\textbf{twenty years} \textbf{before and we were never buddies in} one\textbf{the first place}                                           \\
\multicolumn{1}{c}{}                     & NeuSpeech w/ pt   &  \textbf{I seen him since high school maybe twenty years before and we were never buddies in the first place} he talked to me since t.                                                                           \\
\multicolumn{1}{c}{}                     & NeuSpeech w/ jt   & \textbf{I seen him since high school maybe twenty years before and we were never buddies in the first place}                                                                                \\
\multicolumn{1}{c}{}                     & eeg-to-text~\cite{wang2022open_aaai_eeg2text}       & \underline{It was a long time since I had last seen him} in the flesh                                                                                                       \\
\multicolumn{1}{c}{}                     & eeg-to-text~\cite{wang2022open_aaai_eeg2text} w/ tf & was the and I \textbf{school} a \textbf{years} ago that he had both close \textbf{the first place}                                                                               \\\cmidrule(l){1-3} 
\multirow{7}{*}{(2)}                     & GT                & My patience was long gone and I was back in the car to warming up when Acres tapped on the window and told me he had found whatever he was looking for               \\
& NeuSpeech         & \textbf{My patience was long gone and I was back in the car}. But when I heard that many of you were \textbf{looking for} whatever it was, but what about this?                        \\
& NeuSpeech w/ tf   & \textbf{My patience was long gone and I was back in} a\textbf{the car}.\textbf{to warming up when Acres} was\textbf{tapped on the}the \textbf{window and} opened\textbf{told me he had found whatever he was looking for}. \\
& NeuSpeech w/ pt   & \textbf{My patience was long gone and I was back in the car}.                                                                                                                 \\
& NeuSpeech w/ jt   & \textbf{My patience was long gone and I was back in the car}. The window was looking good when Acres is ongoing on her car and she now has...                                 \\
& eeg-to-text~\cite{wang2022open_aaai_eeg2text}       & \underline{He said} he had no idea how \textbf{long} it would take him to get \textbf{back} home                                                                                                   \\
& eeg-to-text~\cite{wang2022open_aaai_eeg2text} w/ tf & father was running gone I was ready to the dark \underline{drive} up Iacia me the \textbf{window} said me to was a a \textbf{he was looking for}                                                   \\ \cmidrule(l){1-3} 
\multirow{7}{*}{(3)}                     & GT                & Very well said Arthur then take your story to that and let him defend you when no civilized publisher will approach you                                              \\
& NeuSpeech         & \textbf{Very well said Arthur}! Tell me \textbf{your story}, and I'll \textbf{defend} it from \textbf{you when no civilized publisher will approach you}.                                                \\
& NeuSpeech w/ tf   & \textbf{Very well said Arthur}!\textbf{then} that\textbf{take your story to} and\textbf{that and let him defend you} and \textbf{no civilized publisher will approach you} when                                   \\
& NeuSpeech w/ pt   & \textbf{Very well said Arthur then take your story to that and let him defend you when no civilized publisher will approach you} \textbf{very well}                                    \\
& NeuSpeech w/ jt   & \textbf{Very well said}! It was that and we can make sure that it and not \textbf{let him defend you when no civilized publisher will approach you}                                    \\
& eeg-to-text~\cite{wang2022open_aaai_eeg2text}       & It was the first time I had seen him in a long time and it made me very nervous                                                                                      \\
& eeg-to-text~\cite{wang2022open_aaai_eeg2text} w/ tf & little then he the seat and the place go it take it he one man \underline{would you}   \\ \bottomrule                                                                                         
\end{tabular}
    }
    % \vspace{-15pt}
\end{table*}

